Defense against Adversarial Cloud Attack on Remote Sensing Salient Object Detection

Detecting the salient objects in a remote sensing image has wide applications for the interdisciplinary research. Many existing deep learning methods have been proposed for Salient Object Detection (SOD) in remote sensing images and get remarkable results. However, the recent adversarial attack examples, generated by changing a few pixel values on the original remote sensing image, could result in a collapse for the well-trained deep learning based SOD model. Different with existing methods adding perturbation to original images, we propose to jointly tune adversarial exposure and additive perturbation for attack and constrain image close to cloudy image as Adversarial Cloud. Cloud is natural and common in remote sensing images, however, camouflaging cloud based adversarial attack and defense for remote sensing images are not well studied before. Furthermore, we design DefenseNet as a learn-able pre-processing to the adversarial cloudy images so as to preserve the performance of the deep learning based remote sensing SOD model, without tuning the already deployed deep SOD model. By considering both regular and generalized adversarial examples, the proposed DefenseNet can defend the proposed Adversarial Cloud in white-box setting and other attack methods in black-box setting. Experimental results on a synthesized benchmark from the public remote sensing SOD dataset (EORSSD) show the promising defense against adversarial cloud attacks.

==> main <==
\begin{thebibliography}{10}

\bibitem{wang2016salient}
Q.~Wang, J.~Lin, and Y.~Yuan, ``Salient band selection for hyperspectral image
  classification via manifold ranking,'' {\em IEEE Transactions on Neural
  Networks and Learning Systems}, vol.~27, no.~6, pp.~1279--1289, 2016.

\bibitem{zhang2018diverse}
M.~Zhang, W.~Li, and Q.~Du, ``Diverse region-based cnn for hyperspectral image
  classification,'' {\em IEEE Transactions on Image Processing}, vol.~27,
  no.~6, pp.~2623--2634, 2018.

\bibitem{tian2017cross}
Y.~Tian, C.~Chen, and M.~Shah, ``Cross-view image matching for geo-localization
  in urban environments,'' in {\em IEEE/CVF Conference on Computer Vision and
  Pattern Recognition}, pp.~3608--3616, 2017.

\bibitem{zhu2021revisiting}
S.~Zhu, T.~Yang, and C.~Chen, ``Revisiting street-to-aerial view image
  geo-localization and orientation estimation,'' in {\em IEEE/CVF Winter
  Conference on Applications of Computer Vision}, pp.~756--765, 2021.

\bibitem{zou2015deep}
Q.~Zou, L.~Ni, T.~Zhang, and Q.~Wang, ``Deep learning based feature selection
  for remote sensing scene classification,'' {\em IEEE Geoscience and Remote
  Sensing Letters}, vol.~12, no.~11, pp.~2321--2325, 2015.

\bibitem{song2019domain}
S.~Song, H.~Yu, Z.~Miao, Q.~Zhang, Y.~Lin, and S.~Wang, ``Domain adaptation for
  convolutional neural networks-based remote sensing scene classification,''
  {\em IEEE Geoscience and Remote Sensing Letters}, vol.~16, no.~8,
  pp.~1324--1328, 2019.

\bibitem{bruzzone2002adaptive}
L.~Bruzzone and D.~F. Prieto, ``An adaptive semiparametric and context-based
  approach to unsupervised change detection in multitemporal remote-sensing
  images,'' {\em IEEE Transactions on Image Processing}, vol.~11, no.~4,
  pp.~452--466, 2002.

\bibitem{du2019unsupervised}
B.~Du, L.~Ru, C.~Wu, and L.~Zhang, ``Unsupervised deep slow feature analysis
  for change detection in multi-temporal remote sensing images,'' {\em IEEE
  Transactions on Geoscience and Remote Sensing}, vol.~57, no.~12,
  pp.~9976--9992, 2019.

\bibitem{Xia_2018_CVPR}
G.-S. Xia, X.~Bai, J.~Ding, Z.~Zhu, S.~Belongie, J.~Luo, M.~Datcu, M.~Pelillo,
  and L.~Zhang, ``Dota: A large-scale dataset for object detection in aerial
  images,'' in {\em IEEE/CVF Conference on Computer Vision and Pattern
  Recognition}, 2018.

\bibitem{ding2019learning}
J.~Ding, N.~Xue, Y.~Long, G.-S. Xia, and Q.~Lu, ``Learning roi transformer for
  oriented object detection in aerial images,'' in {\em IEEE/CVF Conference on
  Computer Vision and Pattern Recognition}, pp.~2849--2858, 2019.

\bibitem{li2019nested}
C.~Li, R.~Cong, J.~Hou, S.~Zhang, Y.~Qian, and S.~Kwong, ``Nested network with
  two-stream pyramid for salient object detection in optical remote sensing
  images,'' {\em IEEE Transactions on Geoscience and Remote Sensing}, vol.~57,
  no.~11, pp.~9156--9166, 2019.

\bibitem{zhang2020dense}
Q.~Zhang, R.~Cong, C.~Li, M.-M. Cheng, Y.~Fang, X.~Cao, Y.~Zhao, and S.~Kwong,
  ``Dense attention fluid network for salient object detection in optical
  remote sensing images,'' {\em IEEE Transactions on Image Processing},
  vol.~30, pp.~1305--1317, 2020.

\bibitem{gao2022can}
R.~Gao, Q.~Guo, F.~Juefei-Xu, H.~Yu, H.~Fu, W.~Feng, Y.~Liu, and S.~Wang, ``Can
  you spot the chameleon? adversarially camouflaging images from co-salient
  object detection,'' in {\em IEEE/CVF Conference on Computer Vision and
  Pattern Recognition}, 2022.

\bibitem{goodfellow2014explaining}
I.~J. Goodfellow, J.~Shlens, and C.~Szegedy, ``Explaining and harnessing
  adversarial examples,'' {\em arXiv preprint arXiv:1412.6572}, 2014.

\bibitem{gao2021advhaze}
R.~Gao, Q.~Guo, F.~Juefei-Xu, H.~Yu, and W.~Feng, ``Advhaze: Adversarial haze
  attack,'' {\em arXiv preprint arXiv:2104.13673}, 2021.

\bibitem{liao2018defense}
F.~Liao, M.~Liang, Y.~Dong, T.~Pang, X.~Hu, and J.~Zhu, ``Defense against
  adversarial attacks using high-level representation guided denoiser,'' in
  {\em IEEE Conference on Computer Vision and Pattern Recognition},
  pp.~1778--1787, 2018.

\bibitem{zhang2019defense}
H.~Zhang and J.~Wang, ``Defense against adversarial attacks using feature
  scattering-based adversarial training,'' {\em Advances in Neural Information
  Processing Systems}, vol.~32, 2019.

\bibitem{xu2020assessing}
Y.~Xu, B.~Du, and L.~Zhang, ``Assessing the threat of adversarial examples on
  deep neural networks for remote sensing scene classification: Attacks and
  defenses,'' {\em IEEE Transactions on Geoscience and Remote Sensing},
  vol.~59, no.~2, pp.~1604--1617, 2020.

\bibitem{sun2021convolutional}
H.~Sun, Y.~Lin, Q.~Zou, S.~Song, J.~Fang, and H.~Yu, ``Convolutional neural
  networks based remote sensing scene classification under clear and cloudy
  environments,'' in {\em IEEE/CVF International Conference on Computer Vision
  Workshop}, pp.~713--720, 2021.

\bibitem{li2016building}
E.~Li, S.~Xu, W.~Meng, and X.~Zhang, ``Building extraction from remotely sensed
  images by integrating saliency cue,'' {\em IEEE Journal of Selected Topics in
  Applied Earth Observations and Remote Sensing}, vol.~10, no.~3, pp.~906--919,
  2016.

\bibitem{ma2016region}
L.~Ma, B.~Du, H.~Chen, and N.~Q. Soomro, ``Region-of-interest detection via
  superpixel-to-pixel saliency analysis for remote sensing image,'' {\em IEEE
  Geoscience and Remote Sensing Letters}, vol.~13, no.~12, pp.~1752--1756,
  2016.

\bibitem{zhang2018airport}
Q.~Zhang, L.~Zhang, W.~Shi, and Y.~Liu, ``Airport extraction via complementary
  saliency analysis and saliency-oriented active contour model,'' {\em IEEE
  Geoscience and Remote Sensing Letters}, vol.~15, no.~7, pp.~1085--1089, 2018.

\bibitem{liu2019unsupervised}
Z.~Liu, D.~Zhao, Z.~Shi, and Z.~Jiang, ``Unsupervised saliency model with color
  markov chain for oil tank detection,'' {\em Remote Sensing}, vol.~11, no.~9,
  p.~1089, 2019.

\bibitem{dong2019ship}
C.~Dong, J.~Liu, F.~Xu, and C.~Liu, ``Ship detection from optical remote
  sensing images using multi-scale analysis and fourier hog descriptor,'' {\em
  Remote Sensing}, vol.~11, no.~13, p.~1529, 2019.

\bibitem{zhao2015sparsity}
D.~Zhao, J.~Wang, J.~Shi, and Z.~Jiang, ``Sparsity-guided saliency detection
  for remote sensing images,'' {\em Journal of Applied Remote Sensing}, vol.~9,
  no.~1, p.~095055, 2015.

\bibitem{zhang2019saliency}
L.~Zhang, Y.~Liu, and J.~Zhang, ``Saliency detection based on self-adaptive
  multiple feature fusion for remote sensing images,'' {\em International
  Journal of Remote Sensing}, vol.~40, no.~22, pp.~8270--8297, 2019.

\bibitem{zhang2013region}
L.~Zhang and K.~Yang, ``Region-of-interest extraction based on frequency domain
  analysis and salient region detection for remote sensing image,'' {\em IEEE
  Geoscience and Remote Sensing Letters}, vol.~11, no.~5, pp.~916--920, 2013.

\bibitem{zhang2015region}
Y.~Zhang, L.~Zhang, and X.~Yu, ``Region of interest extraction based on
  multiscale visual saliency analysis for remote sensing images,'' {\em Journal
  of Applied Remote Sensing}, vol.~9, no.~1, p.~095050, 2015.

\bibitem{li2020parallel}
C.~Li, R.~Cong, C.~Guo, H.~Li, C.~Zhang, F.~Zheng, and Y.~Zhao, ``A parallel
  down-up fusion network for salient object detection in optical remote sensing
  images,'' {\em Neurocomputing}, vol.~415, pp.~411--420, 2020.

\bibitem{zhang2021salient}
L.~Zhang and J.~Ma, ``Salient object detection based on progressively
  supervised learning for remote sensing images,'' {\em IEEE Transactions on
  Geoscience and Remote Sensing}, 2021.

\bibitem{cong2021rrnet}
R.~Cong, Y.~Zhang, L.~Fang, J.~Li, Y.~Zhao, and S.~Kwong, ``Rrnet: Relational
  reasoning network with parallel multiscale attention for salient object
  detection in optical remote sensing images,'' {\em IEEE Transactions on
  Geoscience and Remote Sensing}, vol.~60, pp.~1--11, 2021.

\bibitem{szegedy2013intriguing}
C.~Szegedy, W.~Zaremba, I.~Sutskever, J.~Bruna, D.~Erhan, I.~Goodfellow, and
  R.~Fergus, ``Intriguing properties of neural networks,'' in {\em
  International Conference on Learning Representations}, 2014.

\bibitem{madry2017towards}
A.~Madry, A.~Makelov, L.~Schmidt, D.~Tsipras, and A.~Vladu, ``Towards deep
  learning models resistant to adversarial attacks,'' in {\em International
  Conference on Learning Representations}, 2018.

\bibitem{carlini2017towards}
N.~Carlini and D.~Wagner, ``Towards evaluating the robustness of neural
  networks,'' in {\em 2017 IEEE symposium on security and privacy (SP)}, 2017.

\bibitem{AA_atack_2020}
F.~Croce and M.~Hein, ``Reliable evaluation of adversarial robustness with an
  ensemble of diverse parameter-free attacks,'' in {\em International
  Conference on Machine Learning}, 2020.

\bibitem{croce2020minimally}
F.~Croce and M.~Hein, ``Minimally distorted adversarial examples with a fast
  adaptive boundary attack,'' in {\em International Conference on Machine
  Learning}, 2020.

\bibitem{andriushchenko2020square}
M.~Andriushchenko, F.~Croce, N.~Flammarion, and M.~Hein, ``Square attack: a
  query-efficient black-box adversarial attack via random search,'' in {\em
  European Conference on Computer Vision}, Springer, 2020.

\bibitem{goodfellow2009measuring}
I.~Goodfellow, H.~Lee, Q.~Le, A.~Saxe, and A.~Ng, ``Measuring invariances in
  deep networks,'' in {\em Conference on Neural Information Processing
  Systems}, 2009.

\bibitem{kanbak2018geometric}
C.~Kanbak, S.-M. Moosavi-Dezfooli, and P.~Frossard, ``Geometric robustness of
  deep networks: analysis and improvement,'' in {\em IEEE Conference on
  Computer Vision and Pattern Recognition}, 2018.

\bibitem{huang2020universal}
L.~Huang, C.~Gao, Y.~Zhou, C.~Xie, A.~L. Yuille, C.~Zou, and N.~Liu,
  ``Universal physical camouflage attacks on object detectors,'' in {\em IEEE
  Conference on Computer Vision and Pattern Recognition}, 2020.

\bibitem{kurakin2016adversarial}
A.~Kurakin, I.~Goodfellow, and S.~Bengio, ``Adversarial examples in the
  physical world,'' {\em International Conference on Learning Representations
  Workshop}, 2017.

\bibitem{lu2017safetynet}
J.~Lu, T.~Issaranon, and D.~Forsyth, ``Safetynet: Detecting and rejecting
  adversarial examples robustly,'' in {\em International Conference on
  Conference on Computer Vision}, 2017.

\bibitem{Mao2019}
C.~Mao, Z.~Zhong, J.~Yang, C.~Vondrick, and B.~Ray, ``Metric learning for
  adversarial robustness,'' in {\em Conference on Neural Information Processing
  Systems}, 2019.

\bibitem{Zhong2019}
Y.~Zhong and W.~Deng, ``Adversarial learning with margin-based triplet
  embedding regularization,'' in {\em International Conference on Conference on
  Computer Vision}, 2019.

\bibitem{shafahi2019adversarial}
A.~Shafahi, M.~Najibi, M.~A. Ghiasi, Z.~Xu, J.~Dickerson, C.~Studer, L.~S.
  Davis, G.~Taylor, and T.~Goldstein, ``Adversarial training for free!,'' in
  {\em Conference on Neural Information Processing Systems}, 2019.

\bibitem{zhang2019theoretically}
H.~Zhang, Y.~Yu, J.~Jiao, E.~P. Xing, L.~E. Ghaoui, and M.~I. Jordan,
  ``Theoretically principled trade-off between robustness and accuracy,'' in
  {\em International Conference on Machine Learning}, 2019.

\bibitem{MART_2020}
Y.~Wang, D.~Zou, J.~Yi, J.~Bailey, X.~Ma, and Q.~Gu, ``Improving adversarial
  robustness requires revisiting misclassified examples,'' in {\em
  International Conference on Learning Representations}, 2019.

\bibitem{wang2021agkd}
H.~Wang, Y.~Deng, S.~Yoo, H.~Ling, and Y.~Lin, ``Agkd-bml: Defense against
  adversarial attack by attention guided knowledge distillation and
  bi-directional metric learning,'' in {\em Proceedings of the IEEE/CVF
  International Conference on Computer Vision}, pp.~7658--7667, 2021.

\bibitem{xie2019feature}
C.~Xie, Y.~Wu, L.~v.~d. Maaten, A.~L. Yuille, and K.~He, ``Feature denoising
  for improving adversarial robustness,'' in {\em IEEE Conference on Computer
  Vision and Pattern Recognition}, 2019.

\bibitem{cohen2019certified}
J.~Cohen, E.~Rosenfeld, and Z.~Kolter, ``Certified adversarial robustness via
  randomized smoothing,'' in {\em International Conference on Machine
  Learning}, 2019.

\bibitem{song2018pixeldefend}
Y.~Song, T.~Kim, S.~Nowozin, S.~Ermon, and N.~Kushman, ``Pixeldefend:
  Leveraging generative models to understand and defend against adversarial
  examples,'' in {\em International Conference on Learning Representations},
  2018.

\bibitem{sun2019adversarial}
B.~Sun, N.-h. Tsai, F.~Liu, R.~Yu, and H.~Su, ``Adversarial defense by
  stratified convolutional sparse coding,'' in {\em IEEE Conference on Computer
  Vision and Pattern Recognition}, 2019.

\bibitem{yuan2020ensemble}
J.~Yuan and Z.~He, ``Ensemble generative cleaning with feedback loops for
  defending adversarial attacks,'' in {\em IEEE Conference on Computer Vision
  and Pattern Recognition}, 2020.

\bibitem{loshchilov2017decoupled}
I.~Loshchilov and F.~Hutter, ``Decoupled weight decay regularization,'' {\em
  arXiv preprint arXiv:1711.05101}, 2017.

\bibitem{das2018shield}
N.~Das, M.~Shanbhogue, S.-T. Chen, F.~Hohman, S.~Li, L.~Chen, M.~E. Kounavis,
  and D.~H. Chau, ``Shield: Fast, practical defense and vaccination for deep
  learning using jpeg compression,'' in {\em Proceedings of the 24th ACM SIGKDD
  International Conference on Knowledge Discovery \& Data Mining},
  pp.~196--204, 2018.

\bibitem{qin2020ffa}
X.~Qin, Z.~Wang, Y.~Bai, X.~Xie, and H.~Jia, ``Ffa-net: Feature fusion
  attention network for single image dehazing,'' in {\em AAAI Conference on
  Artificial Intelligence}, pp.~11908--11915, 2020.

\bibitem{dong2018boosting}
Y.~Dong, F.~Liao, T.~Pang, H.~Su, J.~Zhu, X.~Hu, and J.~Li, ``Boosting
  adversarial attacks with momentum,'' in {\em IEEE Conference on Computer
  Vision and Pattern Recognition}, 2018.

\bibitem{wang2021enhancing}
X.~Wang and K.~He, ``Enhancing the transferability of adversarial attacks
  through variance tuning,'' in {\em IEEE/CVF Conference on Computer Vision and
  Pattern Recognition}, pp.~1924--1933, 2021.

\bibitem{lin2019nesterov}
J.~Lin, C.~Song, K.~He, L.~Wang, and J.~E. Hopcroft, ``Nesterov accelerated
  gradient and scale invariance for adversarial attacks,'' {\em arXiv preprint
  arXiv:1908.06281}, 2019.

\bibitem{qin2019basnet}
X.~Qin, Z.~Zhang, C.~Huang, C.~Gao, M.~Dehghan, and M.~Jagersand, ``Basnet:
  Boundary-aware salient object detection,'' in {\em Proceedings of the
  IEEE/CVF conference on computer vision and pattern recognition},
  pp.~7479--7489, 2019.

\bibitem{qin2020u2}
X.~Qin, Z.~Zhang, C.~Huang, M.~Dehghan, O.~R. Zaiane, and M.~Jagersand,
  ``U2-net: Going deeper with nested u-structure for salient object
  detection,'' {\em Pattern recognition}, vol.~106, p.~107404, 2020.

\end{thebibliography}

